Unbeschr\"ankte Multiplikatoren auf Operatorr\"aumen

We introduce unbounded multipliers on operator spaces. These multipliers generalize both, regular operators on Hilbert C*-modules and (bounded) multipliers on operator spaces. ----- Wir definieren den Begriff eines unbeschr\"ankten Multiplikators auf Operatorr\"aumen. Diese Multiplikatoren verallgemeinern sowohl regul\"are Operatoren auf Hilbert-C*-Moduln als auch (beschr\"ankte) Multiplikatoren auf Operatorr\"aumen.

==> MathPreamble2.tex <==
% Vorspann für mathematische Texte

\usepackage{german}
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
%\usepackage{t1enc}   % veraltet, benutze \usepackage[T1]{fontenc}
%\usepackage{a4wide}  % am 11.11.03 auskommentiert
\usepackage{amsmath}  % wird für \begin{cases} benötigt
\usepackage{amsthm}
%\usepackage{makeidx}
\usepackage{exscale}   % verbessert die Darstellung mathematischer Formeln
\usepackage{enumerate}
\usepackage{bbm}    % \mathbbm ersetzt \mathbb (z.B. für ein besseres R für die reellen Zahlen)
%\usepackage[active]{srcltx}  % für WinEdt zur Inversen Suche; mit MiKTeX nicht notwendig, 
% benutze die Kommandozeile --src
%\usepackage{layout}  % zeigt das Seitenlayout mittels \layout mit den Maßen an
\usepackage{xspace}  % Space after command names (DPC)
%aus Xenias Datei MathDef.tex
\RequirePackage{amssymb}
\RequirePackage{latexsym}
%\RequirePackage{tabularx}

\hyphenation{Ba-nach-al-ge-bra}

\DeclareMathOperator{\supp}{supp}   % Support (Träger)
\DeclareMathOperator{\Spur}{Spur}   % die Spur
\DeclareMathOperator{\Id}{Id}       % die Identität
\DeclareMathOperator{\Def}{Def}     % der Definitionsbereich einer Relation
\DeclareMathOperator{\Bild}{Bild}   % der Bildbereich einer Relation
\DeclareMathOperator{\Kern}{Kern}   % der Kern einer Abbildung
\DeclareMathOperator{\vdim}{dim}    % die Dimension eines Vektorraumes

